Wake-Based Locomotion Gait Design for Aerobat

Flying animals, such as bats, fly through their fluidic environment as they create air jets and form wake structures downstream of their flight path. Bats, in particular, dynamically morph their highly flexible and dexterous armwing to manipulate their fluidic environment which is key to their agility and flight efficiency. This paper presents the theoretical and numerical analysis of the wake-structure-based gait design inspired by bat flight for flapping robots using the notion of reduced-order models and unsteady aerodynamic model incorporating Wagner function. The objective of this paper is to introduce the notion of gait design for flapping robots by systematically searching the design space in the context of optimization. The solution found using our gait design framework was used to design and test a flapping robot.

==> unused.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/aerobat_ks_joint_id.pdf}
    \caption{The linkage model of the Aerobat's KS which consists of 7 linkages and 10 joints, labeled $L_i$ and $J_j$, respectively. $J_1$, $J_5$, and $J_8$ positions are fixed on the body while $L_1$ represents the gear/crank moment arm. The angle of joint $i$ ($\theta_i$) is defined with respect to the body's $y$-axis, e.g. shown in this image is the angle of joint 5 ($\theta_5$).}
    \label{fig:ks_linkages_details}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/linkages_length.pdf}
    \caption{Linkage dimensions of the Aerobat's KS mechanism. There are 16 linkage parameters and 6 joint positions ($J_1$, $J_5$, and $J_8$) which determine the resulting flapping trajectory.}
    \label{fig:aerobat_linkages_dimensions}
\end{figure}



\begin{table}[t]
    %\vspace{0.1in}
    \centering
    \caption{Sensitivity Analysis of the Armwing KS Parameters}
    %\vspace{-0.1in}
    \begin{tabular}{c | c c c c c}
    \toprule
    $\bm{q}$ & $A_s$ & $A_e$ & $M_s$ & $M_e$ & $\Delta \theta$ \\
    \midrule
    $l_1$    & 200   & 205   & -9.00 & -124  & 4.32$\cdot 10^{3}$ \\
    $l_{2a}$ & 6.97  & -137  & -204  &  244  & -1.54$\cdot 10^{3}$ \\
    $l_{2b}$ & 0     & 183   & 0     & -306  & 0 \\
    $l_{2c}$ & 0     & 115   & 0     & -193  & 0 \\
    $l_{3a}$ & 0     & -1.81 & 0     &  22.3 & -2.26$\cdot 10^{3}$ \\
    $l_{3b}$ & -124  & -67.9 & -65.8 & 119   & 1.06$\cdot 10^{4}$ \\
    $l_{3c}$ & -111  & 148   & 90.2  & -263  & 0 \\
    $\alpha_3$ & 0   & 1.26  & 1.00  & -2.11 & 0 \\
    $l_{4}$  & 0     & 220   & 0     & -367  & 1.56$\cdot 10^{4}$ \\
    $l_{5a}$ & 0     & -68.5 & 0     & -20.4 & -1.33$\cdot 10^{4}$ \\
    $l_{5b}$ & 0     & -217  & 0     & 356   & -8.88$\cdot 10^{3}$ \\
    $l_{5c}$ & 0     &  3.11 & 0     & -8.70 & -1.43$\cdot 10^{3}$ \\
    $l_{5d}$ & 0     & -22.3 & 0     &  48.4 &  0 \\
    $l_{6}$  & 0     &  22.5 & 0     & -49.2 &  0 \\
    $l_{7b}$ & 0     & -28.7 & 0     &  42.9 &  0 \\
    $l_{7c}$ & 0     & -12.2 &  0    & -10.1 &  0\\
    $p_{1y}$ & 7.50  & -11.2 & -158  & 69.0  &  3.24$\cdot 10^{3}$\\
    $p_{1z}$ & 4.78  &  131  & -123  & -189  &  7.59$\cdot 10^{3}$\\
    $p_{5y}$ & -7.04 &  157  &  159  & -203  &  -6.97$\cdot 10^{2}$\\
    $p_{5z}$ & -4.83 &  78.1 &  123  & -190  &  0\\
    $p_{8y}$ & 0     & -147  &  0    &  135  &  -1.55$\cdot 10^{3}$\\
    $p_{8z}$ & 0     & -208  &  0    &  378  &  -1.09$\cdot 10^{4}$\\
    \bottomrule
    \multicolumn{6}{l}{Note: units are rad/m or rad/rad (for $\alpha_3$). \Tstrut}
    \end{tabular}
    %\vspace{-0.1in}
    \label{tab:sensitivity}
\end{table}


\begin{table}[t]
    %\vspace{0.1in}
    \centering
    \caption{Sensitivity Analysis of the Wing Mechanism Parameters}
    %\vspace{-0.1in}
    \begin{tabular}{c | c c c c c}
    \toprule
    $\bm{q}$ & $A_s$ & $A_e$ & $M_s$ & $M_e$ & $\Delta \theta$ \\
    \midrule
    $l_1$ & \textbf{19.7} &\textbf{ 47.7} & -1.40 & -3.47 & \textbf{18.6} \\
    $l_2$ & -2.79 & 2.48 & 9.86 & -28.6 &  -4.71 \\
    $l_{3a}$ & -2.94 & -17.7 & -10.2 &  30.9 & -1.23 \\
    $l_{3b}$ &  -1.51 &  8.85 & 11.1 & \textbf{-30.97} & -5.21 \\
    $l_{3c}$ &  1.87 & 2.93 & -2.06 & 5.74 & 0 \\
    $l_4$ &   1.83 & -8.14 & \textbf{-11.3} &  31.6 & 3.81 \\
    $l_{5a}$ & -5.49 &  -19.8 &   -6.83 &  22.5  & -5.37 \\
    $l_{5b}$ & -7.47 &  -6.59 &   7.79 & -21.5 &  -7.89 \\
    $\alpha_5$ & 0  & 68.5  & 57.3 & -163 & 0 \\
    $p_{4y}$ & -6.96 &  -6.22 &   8.56 & -21.4226 & -12.4 \\
    $p_{7x}$ & -2.36 &   7.40 &  11.0 & -30.3708 &  -6.19 \\
    $p_{7y}$ &  4.22 &  11.3  &  1.28 &  -9.05 &  5.18 \\
    $\phi_{0}$ &  -2.2$\cdot 10^{-4}$ & -2.3$\cdot 10^{-4}$ & -4.3$\cdot 10^{-4}$ & -2.5$\cdot 10^{-4}$ & 0 \\
    $l_6$ & 0 &  \textbf{-23.7} & 0&  14.2 &  \textbf{-20.8} \\
    $l_7$ & 0 &   8.69 &  0 &  \textbf{-24.9} &    1.5\\
    $l_{8a}$ & 0 &   12.3 &  0 &  -15.0 &    5.4\\
    $l_{8b}$ & 0 &   -9.5 &  0 &   15.0 &  -5.14\\
    $l_{8c}$ & 0 &  -1.14 &  0 &  -14.0 &   -5.4\\
    $l_9$ & 0 &    6.07 &  0 &  -20.9 &   -2.0\\
    $l_{10a}$ &  0 &    10.8 &  0 &  -16.5 &    7.2\\
    $l_{10b}$ &  0 &    4.36 &  0 &   11.7 &   7.71\\
    $l_{10c}$ &  0 &   -2.37 &  0 &  0.045 &  0.514\\
    $l_{10d}$ &  0 &   -1.08 &  0 &    2.5 &      0\\
    $l_{11}$ &  0 &    1.01 &  0 &  -2.77 &      0\\
    $l_{12a}$ &  0 &    -1.3 &  0 &   2.51 &      0\\
    $l_{12b}$ &  0 &  -0.434 &  0 &  -1.08 &      0\\
    $p_{12y}$ & 0 &   -6.09 &  0 &   10.6 &   -3.6\\
    $p_{14x}$ & 0 &   -6.51 &  0 &   15.5 &   2.28\\
    $p_{14y}$ & 0 &   -4.28 &  0 &   16.3 &      0\\
    $\Delta \phi$ & 0 &   117.0 &  0 &   12.1 &      0\\
    \bottomrule
    \multicolumn{6}{l}{Note: units are rad/mm for length or position and rad/rad for angles. \Tstrut}
    \end{tabular}
    %\vspace{-0.1in}
    \label{tab:sensitivity}
\end{table}
